MROS: Runtime Adaptation For Robot Control Architectures

Known attempts to build autonomous robots rely on complex control architectures, often implemented with the Robot Operating System platform (ROS). Runtime adaptation is needed in these systems, to cope with component failures and with contingencies arising from dynamic environments-otherwise, these affect the reliability and quality of the mission execution. Existing proposals on how to build self-adaptive systems in robotics usually require a major re-design of the control architecture and rely on complex tools unfamiliar to the robotics community. Moreover, they are hard to reuse across applications. This paper presents MROS: a model-based framework for run-time adaptation of robot control architectures based on ROS. MROS uses a combination of domain-specific languages to model architectural variants and captures mission quality concerns, and an ontology-based implementation of the MAPE-K and meta-control visions for run-time adaptation. The experiment results obtained applying MROS in two realistic ROS-based robotic demonstrators show the benefits of our approach in terms of the quality of the mission execution, and MROS' extensibility and re-usability across robotic applications.

==> componentfailures.tex <==
\subsubsection{Management of component failures at run-time \\ (Dual-arm manipulator)}
%\subsubsection*{Dual-arm mobile manipulator}

The experimental setup involved a dual-arm mobile manipulator, consisting of a ABB YuMi mounted on a Ridgeback omnidirectional platform and an Intel Real sense camera (Figure~\ref{fig:pyramid}).
We focus on performance of the different control schemes in different operational contexts as a key non-functional property here. 
\begin{itemize}
    \item Scenario 1: manipulator does not detect the workstation tag.
    \item Scenario 2: manipulator can operate with only one arm.
 %   \item Scenario 3: laser sensor fails (a mobile robot).
\end{itemize}

The first scenario demonstrates the MROS ability to recover a function that requires multiple components. When the workstation tag is not detected, the robot needs to calibrate its pose with respect to a
QR tag visible on top of the workstation. Due to changing lightning
conditions, the algorithm may fail to detect the tag. The MROS meta-controller can switch between alternative configurations of
the camera parameters that work better under different lighting, to
detect the tag. The second scenario demonstrates the MROS controller’s ability
to recover from an error by realising an alternative set of functions
to perform the task goal with degraded performance. We inject a
failure by blocking one of the robot’s arms.
%The robot builds a pyramid from two piles of blocks. For that it first calibrates its position with respect to the workstation using a tag and its camera. Then it performs the pick-and-place motions to build the pyramid using both arms and prior knowledge about the position of the piles, the blocks sizes and desired position for the pyramid.


%We encoded two scenarios: 
%focus on performance of the different control schemes in different operational contexts as a key non-functional property here.  There are three scenarios:
%
%\begin{itemize}
 %   \item Scenario 1: manipulator does not detect the workstation tag.
  %  \item Scenario 2: manipulator can operate with only one arm.
 %   \item Scenario 3: laser sensor fails (a mobile robot).
%\end{itemize}
%
%The first scenario aims to demonstrate the MROS ability to recover a function that requires multiple components. When the workstation tag is not detected, the robot calibrates its pose with respect to a QR tag visible on top of the workstation. Due to changing lightning conditions, the algorithm may fail to detect the tag. The MROS meta-controller switches between alternative configurations of the camera parameters that work better under different lighting, to detect the tag.

%The second scenario demonstrates the MROS controller's ability to recover from an error by realising an alternative set of functions to perform the task goal with degraded performance. It may happen that one of the arms is disabled due to a collision trigger, but the robot is still allowed to moved the other arm and the mobile base. In this case, the metacontrol reconfigures the Yumi to use only one arm,
%(if the collision is safe for further operation, i.e. at a certain min height over the table), 
%for which the robot needs to re-position itself with respect to the workstation. We injected a failure by blocking one of the robot's arms.  MROS identifed the component error and used the functional architecture model to find an alternative variant that uses only the single available arm. %Since the task can no longer be completed with the remaining arm (the wooden blocks are out of range),  MROS effects a change of control algorithm: the platform has to move in order to bring the functioning arm in the range of the block, and complete the task. 
%This results in augmented reliability of the overall system.








==> experimentalsetup.tex <==
 
 %\subsubsection{Management of component failures at and quality attributes at run-time (mobile robot in a factory)}
 
 
 We propose a systematic experimental setup to evaluate the feasibility of the MROS solution at runtime. In order to ensure a comprehensive and consistent experimental setup,
we follow the Goal-Question-Metric method \cite{caldiera1994goal}.

%We designed a reusable experimental framework to evaluate system's runtime adaptation. 
Our goal is to evaluate if MROS is a feasible solution at runtime that improves system and mission performance.
We refine this goal into the following research questions:
\begin{itemize}
\item \textbf{(RQ1)}: \emph{Does MROS improves system and mission robustness in the context of component failures?}%\carlos{use the same structure for both questions, here the context is missing.}} 
\item \textbf{(RQ2)}: \emph{Does MROS improves system and mission performance in the context of component failures and system quality concerns?} 
%We investigate if the MROS framework is able to effective control violation of system qualities and component failures at runtime and is MROS able to improve mission performance.
\end{itemize}


%  implementation of MROS with respect to its management of component failures at runtime.
%Can modelbased intelligent reconfiguration improve mission performance for
%robot systems? Can it address component failures at runtime? Can it
%manage quality concerns at runtime

\subsubsection{Study 1: Manipulation Task}
\carlos{use the same structure for both set ups as much as possible. Study 2 is in the context of a navigation scenario, what is teh context for study 1?}
To address \textbf{(RQ1)}, we did a study on the ABB YuMi dual-arm manipulator \label{sec:yumi} to demonstrate two scenarios: 
\begin{itemize}
\item (i) Scenario 1: manipulator does not detect the workstation tag;
\item (ii) Scenario 2: manipulator can operate with only one arm.
\end{itemize}
 %   \item Scenario 3: laser sensor fails (a mobile robot).
The first scenario aims to demonstrate the MROS ability to recover a function that requires multiple components (increased mission robustness). The  second scenario demonstrates the MROS controller’s ability to recover from  an  error  by  realising  an  alternative  set  of  functions  to perform  the  task  goal  with  degraded  performance (increased system robustness).  We  inject a failure by blocking one of the robot’s arms.


\subsubsection{Study 2: Navigation Task}


To address RQ2,% how the MROS approach  addresses component failures and  quality attribute concerns we designed the following experiment. 
we compared our \textit{MROS} solution to a benchmark system \textit{Base}\carlos{Base, benchmark, baseline are multiple words to refer to the same thing, I would stick to Baseline, with capital as a name for that particular system} with respect to its mission success, component failure and quality concerns 
%performance, safety,  energy-efficiency and component failure 
in the context of a navigation scenario. % We make comparison between two systems:

\emph{Base Benchmark System.~} 
We developed a baseline system based on the standard Navigation Stack of ROS navigating between two locations. \carlos{here a confusion raises, because it looks like that the baseline contains 30 configurations}We implemented 30 system configurations. A system configuration in our experimental setup is defined through a variation of two components: (laser) and (kinect) and different setup of the 7 parameters of the \textit{move\_base} component Figure~\ref{fig:rosgraph}. Some parameters are dependent to each other, so they can be devised if one of them is defined. For the purpose of our experimental setup, we selected 3 main \textit{move\_base} parameters\carlos{I find it confusing that there are explanations for both choosing 7 and 3 parameters, what is the number of parameters relevant for the content of the paper?}, that are independent on each other, more specifically: (i) a parameter that inflates the obstacles the robot perceives in order to regulate the minimal distance to the closest obstacle (\textbf{inflation\_radius}); (ii) a parameter that determines the maximum velocity with which the robot can perform movement (\textbf{max\_vel}), (iii) and a parameter that determines the rate to run the robot's control loop (\textbf{controller\_frequency}). 
%For each of them we assigned 3 values, resulting in 27 different system configurations.

%\begin{figure*}[t]% [__ fig:mapek
%\begin{center}
    

 %   \includegraphics[width=0.9\textwidth]{ROS1Navigation.png}

 %   \vspace{-1mm}
%
  %  \caption{ROS Navigation Stack}%
   
   % \label{fig:nav_stack}


    %\vspace{-2mm}
%\end{center}
%\end{figure*}

% \begin{table}[t]

%   \renewcommand{\arraystretch}{1.22}
%   \begin{tabularx}{\linewidth}{%
%       >{\small\hspace{-2mm}}p{24mm}
%       >{\small\raggedright}X
%       >{\small}c
%       >{\small}c
%       >{\small}c
%       >{\small}c
%     }

%       \textbf{Parameter Name}
%     & \textbf{Description}
%     & \textbf{\clap{Unit}} & \clap{$V_1$} & \clap{$V_2$} & \clap{$V_3$}\\
%     \midrule
%     controller\_frequency (\rlap{cf)} & Rate to run the control loop  & Hz & 15	& 20	& 25 \\
%     planner\_frequency (pf) & Rate to run global planning loop & Hz & 3 & 4	& 5 \\
%     update\_frequency\_g (\rlap{gf)} & Rate to update global map & Hz & 3 & 4	& 5 \\
%     update\_frequency\_l (\rlap{lf)} & Rate to update local map & Hz & 7.5 & 10	& 12.5 \\
%     max\_vel (max\_v) & The maximum allowed base velocity & \clap{$m/s$} & 0.3 & 0.5	& 0.75 \\
%     accel\_lim (a) & The acceleration limit of the robot & \clap{$m/s^2$} & 3.6 & 6	& 9 \\
%     inflation\_radius (r)  & The radius to which the map inflates obstacle cost values & $m$ & 0.5 &	0.65 &	0.8 \\

%     \midrule

%   \end{tabularx}

%   \smallskip

%   \caption{ROS system Parameters for the move\_base node}%
%   \label{tab:confspace}

% \end{table}


\emph{MROS System.~} In the MROS implementation of the system, the MROS Meta-controller runs on top of the baseline, performing run-time analysis and making decisions on when and how to switch to a different system configuration. So, to navigate to the target location the system can additionally self-adapt the robot behaviour by changing its system configurations.

Detailed information about the independent variables of our experiment are provided bellow.  The independent variables are split in two sets:
%
\begin{itemize}

  \item \emph{System parameters:} (i) main ROS global configuration parameters (inflation\_radius, max\_vel, controller\_frequency) 
  
  %(\cref{tab:confspace}).

  \item \emph{Contingency types:} (i) Cluttered context; (ii) Unexpected increase in power usage; (iii) Component failure (discussed bellow).

\end{itemize}
%
During a mission execution, a variation of the aforementioned contingency types can happen. Here, we briefly describe them:
\begin{enumerate}

    \item  \emph{Cluttered environment:} the environment contains a  set of new obstacles unknown to the robot (they are not in the map it uses for navigation) in randomized positions. 
   % The environment includes  a set of unexpected obstacles at run-time. These obstacles are not part of the given map that the robot uses to navigate to the goal. 
     
    Based on the number of obstacles, %and the relative positioning between them, 
    we identify three contingency levels: low (inject 3 new obstacles), medium (inject 8 new obstacles), and high (inject 20 new obstacles).

    \item \textit{Unexpected increase in power consumption:} This contingency might be a result of a sticky surface, a slope, some problem with the wheels, or activation of a new sensor that consumes more power. We also quantify this contingency in three levels: 20\%, 40\%, and 60\% increase in power consumption
    
    \item \textit{Component failure:} We inject a failure in the laser sensor by killing its driver ROS node at run-time.

\end{enumerate}
%
For each run, we investigate how the MROS solution compares to Base in terms of an effective control of system qualities violation, component failures handling and mission performance. A run consists of an initial \emph{launch system configuration C} and a \emph{perturbation P}. We selected 10 initial launch configurations out of 30 that showed the best expected performance in a set of preliminary tests. %Those configurations have been presented in \cref{tab:confspace}.
%is important to note that the set of initial launch configurations C in the system parameters is based on their expected value regarding to each quality attribute. 
A perturbation models a sequence of raised contingencies within a mission. Each perturbation $P$ is represented by a tuple $\langle iv_1, iv_2, iv_3\rangle$, where we assign the contingency specific values to each independent variable within the tuple. More specifically,  $iv_1$ can receive values corresponding to the first type of contingency (cluttered environment): <no contingency, low, medium, high>,  $iv_2$ receives values corresponding to the second type of contingency (increased level of power consumption):
<no\_contingency, 20\%, 40\%, 60\%>, while  $iv_3$ is a boolean that provides information if a laser failure is injected. 



%\begin{table}[t]
%\renewcommand{\arraystretch}{1.22}
%\small
%\begin{center}
%\begin{tabularx}{.66\linewidth}{Xp{1cm} c c  c}
%  \textbf{Conf.} & \textbf{cf} & \textbf{max\_v} & $ r $\\
% \midrule
%C1 &  15	& 0.3	& 0.8 \\
%C2 & 15 & 0.75	& 0.5 \\
%C3 & 20 & 0.3	& 0.8 \\
%C4 & 20 & 0.5	& 0.65 \\
%C5 & 20 & 0.5 & 0.65 \\
%C6 & 25 & 6	& 9 \\
%C7 & 25  &	0.75 &	0.5 \\
%  \midrule
%  \end{tabularx}
%  \end{center}

%  \smallskip

%  \caption{Initial system configuration setup}%
%  \label{tab:confspace}

 % \vspace{-3mm}

%\end{table}


We measure the following dependent variables on the Baseline and the MROS systems for each run:\carlos{I think we need to briefly motivate analyzing these variables, at least those not directly related with the RQs: CPU, memory usage... maybe this results in a modification of the RQs}
%
\begin{itemize}
  \item \textit{Mission success.} A mission is successful if all of following conditions are fulfilled: (i) the robot reaches its goal; (ii) the average safety risk during a run is bellow 0.4;\carlos{I think ii) is redundant with iii) and would remove ii)} (iii) the robot is bellow the safety risk level in more than 95 percent of the mission; (iv) the robot is bellow the energy-consumption level  in more than 90 percent of the mission.     
  \item \textit{Percentage of time} the mission is above safety threshold;
  \item \textit{Percentage of time} the mission is above energy consumption level;
  \item \textit{time to complete} the mission
  \item \textit{memory consumption};
  \item \textit{CPU usage};
  %safety risk level per run is above the threshold for less than 5 percent of the runthe percentage of the time the mission is above a safety threshold 
\end{itemize}
%


==> extensibility.tex <==
 \noindent
 We analyze how the MROS framework supports system extensibility in the context of a mobile robot navigating in a factory scenario with respect to which aspects should one extend in the application:  (i) to capture new components added to the system; (ii) to capture new quality attributes to be monitored.

 \subsubsection{Add new components}

 In the case of the mobile robot, the kinnect component was added so the robot is able to continue the task even if the laser fails. To represent the scenario of a laser failure,  we extended the number of system variants by adding new configurations that contain the kinnect component.  In this case, we used the RosModel tools to model 3 new configurations which corresponds to 30 different variants in total.
 For monitoring, we did not need to add new observer models, because the current tooling allows component failures to be captured.  For analysis and planning, we used the model-to-model transformation that automatically generates the updated knowledge base. Finally, the ROSModel tooling allows automatically generation of available re-configurable actions.
 Hence, to add a new component we only needed to add the new configurations in the ROSModel.


 \subsubsection{Capture new quality attributes}
 In the case, of the mobile robot navigating in a factory, we extended the application scenario by capturing new system quality: energy-efficiency. For monitoring, we developed an observer for energy-efficiency that calculates energy at run-time.
 %For \emph{monitoring}, we developed observer models for safety and energy and component failure.  Safety at run-time was modeled based on the collision risk\,\cite{chung2009safe}.  In this regard, we calculate a breaking distance of the robot before hitting an obstacle \emph{d\_break} and the distance from the current location of the robot to the closest obstacle in its direction $P$.  If the robot is at least \emph{d\_break} distance from the closest obstacle, runtime safety is always 1. As the robot approaches the closest obstacle, safety at run-time is computed as $\nicefrac{P}{\text{\emph{d\_break}}}$.
 Energy at run-time was computed based on a energy model that simulates the power consumption of a robot. The energy model computes the instantaneous \emph{power\_load} of the robot using a set of information like current controller frequency, velocity, acceleration etc.
\looseness=-1

For analysis and planning, we extended the knowledge base with new information about the energy-efficiency of each system configuration. Finally, the ROSModel tooling allows automatically generation of available re-configurable actions. Hence, to capture a new system quality, we only needed to add a corresponding observer and extend the knowledge base by adding information for the energy-efficiency for each system configuration.


==> mobilebase.tex <==
%\section{Case Studies}%
%\label{sec:cases}




%\subsubsection*{Models for design}

%In this use case, we used the design models to build the MROS runtime models for adaptation (the knowledge base).  We analyzed the existing software application for the mobile manipulator and its possible variants with the \emph{ISE\&PPOOA} methodology\,\cite{Fernandez-2019} to obtain the conceptual representation of its functional architecture variants \cref{fig:arch-model}. We captured this model using the TOMASys ontology to build the knowledge base for the meta-controller.

%\subsubsection*{Runtime adaptation}

%For \emph{monitoring} we developed a proof of concept \emph{rosgraph\textunderscore monitor} that allowed mapping component errors in the deployed configurations to the corresponding architectural variant.  For \emph{execution} (reconfiguration) we developed a proof of concept \emph{rosgraph\textunderscore manipulator} mapping of configurations to basic actions that reconfigure the system by killing and launching the relevant ROS nodes.  For \emph{analysis and planning} we used the MROS meta-controller as a re-usable component.



%\darko{Factory Case Study}
%


==> motivatingexample.tex <==
\section{Dual-Arm Mobile Manipulator}
%\subsection{Dual-Arm Mobile Manipulator}% [__
\label{sec:yumi}

\begin{figure}[t]% [__ fig:pyramid

    \includegraphics[
      width=\columnwidth,
      clip,
      trim=0mm 60mm 0mm 10mm
    ]{pyramid.png}

    \vspace{-1mm}

    \caption{YuMi, a dual-arm mobile manipulator at the workstation, attempting to build a pyramid of wooden bricks}%
    \label{fig:pyramid}

    \vspace{-3mm}

\end{figure}
% __]
https://docs.google.com/spreadsheets/d/1LPQIlu0n-PzByPWB4JnenM2dnW_Z5rZI9qogkRpXmUU/edit#gid=2055630334
The mobile manipulator (\cref{fig:pyramid}) is located at a workstation, where it needs to perform a manipulation task \textemdash it needs to build a pyramid out of wooden bricks. To ensure higher robustness than a single robot arm without ability to relocate, we use a YuMi\footnote{https://new.abb.com/products/robotics/collaborative-robots/irb-14000-yumi} dual-arm manipuplator. The two arms provide architecture configuration variability to perform the task using both arms or only one. The YuMi stands on a Clearpath Ridgback platform\footnote{https://clearpathrobotics.com/ridgeback-indoor-robot-platform/} that provides the mobility capability required to reach all the bricks when using only one arm, and has an additional Intel Realsense camera to locate the bricks and a QR-based tag for calibration in the workcell.

The control architecture for this case study consists of ROS components that implement the different functionalities %in the functional architecture variants (see \cref{fig:arch-model}), 
namely: \emph{Pick\&Place bricks}, \emph{Move position} within workstation, \emph{Calibrate position in workcell}, \emph{Locate calibration tag}, \emph{Detect tag} in the camera images.
%The context variability in this case study is 
The presence of humans in the workcell introduces new challenges. Since YuMi is a collaborative robot it needs to ensure a safe interaction. 
We use this case study to introduce our MROS framework.



\begin{figure}[t]% [__ fig:arch-model

  \begin{center}

    \includegraphics[
      width=.8\columnwidth,
    ]{models21_tomasys_abb.pdf}

  \end{center}

  \vspace{-1mm}

  \caption{The model of the functional architecture variants for building a pyramid}%
  \label{fig:arch-model}
% URL OLD: https://app.diagrams.net/#G1iEAGOTXQZsLJEHPn9lwlAHgWbDHgojlK
% URL NEW: https://app.diagrams.net/#G1kj22g_1lPcQWfpd6ehO2MkNeJgLfQGhn  
  \vspace{-3mm}

\end{figure}
% __]

==> results.tex <==
\subsubsection{Study 1: Manipulation Task.}
\carlos{this subsubsection for stufy 1 requires some rewriting imo. I thinks we should present the experimental setup and the results for a demonstrator together, to have better flow.}
The robot builds a pyramid from two piles of blocks. %For that it first calibrates its position with respect to the workstation using a tag and its camera. Then it performs the
%pick-and-place motions to build the pyramid using both arms and prior knowledge about the position of the piles, the blocks sizes and desired position for the pyramid. It may happen that one of the arms is disabled due to a collision trigger, but the robot is still allowed to moved the other arm and the mobile base. %In this case, the metacontrol reconfigures the Yumi to use only one arm (if the collision is safe for further operation, i.e. at a certain min height over the table), for which the robot needs
%to re-position itself with respect to the workstation. Since the task can no longer be completed with the remaining arm  (the  wooden  blocks  are  out  of  range),  MROS  effects  a change of control algorithm: the platform has to move in order to  bring  the  functioning  arm  in  the  range  of  the  block,  and complete the task. This results in augmented reliability of the overall system.
%The first scenario demonstrates the MROS ability to recover a function that requires multiple components. 




\begin{leftbar}

\noindent We conclude that the MROS solution is able to effectively handle component failures and deliver the expected behavior in real-time.
%, generically (using a reasoner and models).

\end{leftbar}

\subsubsection{Study 2: Navigation Task.}
\carlos{check repetition from previous sections in teh first two sentences}
We run our experimental setup on a navigation mission. The mobile robot is placed at a given starting location and it needs to navigate to another workstation using the ROS Navigation stack. An example of the route during one mission is shown in Figure~\ref{fig:nav_mission} in which the starting position is located at the Bottom-Left of the map (-4.5; -7.0) while the goal location is at the Top-Right (8.5; 7.0). In our experimental setup, we considered 7 points for starting and end positions. Moreover, we considered 10 initial system configurations and 32 treatments. In total, we performed $N=2*10*32*27*26*=449 280$ runs for the experiment (MROS and BASE).

\begin{figure}[t]% [__ fig:mapek

    \includegraphics[width=0.9\columnwidth]{exampleRoute.png}

    \vspace{-1mm}

    \caption{Example navigation mission: The route of the mobile manipulator during one mission is shown in red.}%
    \label{fig:nav_mission}


    \vspace{-2mm}

\end{figure}
\carlos{Isn't the following paragraph a repetition?}
For what concerns the management of quality concerns at run-time, we decided to measure the time the system violates a certain quality's attribute constraint. In this context, we specified constraints for safety and energy and monitored how well the system performs the missions under a variation of contingencies.

\Cref{fig:s_violation} shows the average number of times the two systems Base and MROS were performing under the safety threshold of 0.4. It is interesting to note that independently of the level of cluttered environment (number of obstacles in this case), the MROS system always outperforms the base system.  The average time that MROS violates the safety threshold is significantly reduced.  More interestingly, we notice that when the environment is highly cluttered, MROS plays an important role and reduces the violation of the safety constraint from 1.8 to 0.45 seconds.  We have a similar trend for low cluttered environment, where we can observe that MROS reduces the violation from 1.8 to 0.4 seconds.

\begin{figure}[t]% [__ fig:mapek

    \includegraphics[width=\columnwidth]{chart_safety_constraints.pdf}

    \vspace{-1mm}

    \caption{Safety Constraint Violation}%
    \label{fig:s_violation}

    \vspace{-2mm}

\end{figure}

\begin{figure}[t]% [__ fig:mapek

    \includegraphics[width=\columnwidth]{chart_energy_constraints.pdf}

    \vspace{-1mm}

    \caption{Energy Constraint Violation}%
    \label{fig:e_violation}

    \vspace{-2mm}

\end{figure}

\begin{figure}[t]% [__ fig:mapek

    \includegraphics[width=\columnwidth]{chart_mission_time.pdf}

    \vspace{-1mm}

    \caption{Average mission time}%
    \label{fig:time_difference}

    \vspace{-3mm}

\end{figure}

\Cref{fig:e_violation} shows the average time for both systems, Base and the system with MROS, when performing above the energy threshold of 0.7. It is interesting to note that MROS performs better in all the cases. The biggest difference can be noted by a 50\% energy increase, where the result shows that MROS manages to reduce the violation of the energy constraint from 2.46 to 0.65.  Overall, the data shows that MROS has similar results for all variations in energy increase i.e.\ it was able to restrict the violation slightly above 0.5 seconds for all different variations in energy increase.


For what concerns the mission performance, we measured the average time to complete the mission. Figure~\ref{fig:time_difference} shows the average increase in mission completion time when the system uses MROS.\@ For two out of the seven initial launch systems configurations MROS completes the mission faster than Base, while for three other configurations MROS has only a 5\% increase in the mission completion time. Overall, the average mission completion time for Base is 89.18s, while for a system using MROS 93.93s. That means there is a increase in the overall mission time, is the cost for the improvement on the quality parameters (energy consumption and safety).  This is expected as conserving energy puts the robot in a slower mode, and so do more dense obstacles.

\begin{leftbar}

\noindent We conclude that model-based intelligent reconfiguration does improve mission performance for robot systems measurably, managing quality concerns such as safety and energy.

\end{leftbar}



==> reusability.tex <==
\subsubsection{Dual-Arm Manipulator}
In the dual-arm manipulator case study, we used the design models to build the MROS runtime models for adaptation (the knowledge base).  We analyzed the existing software application for the mobile manipulator and its possible variants with the \emph{ISE\&PPOOA} methodology\,\cite{Fernandez-2019} to obtain the conceptual representation of its functional architecture variants as shown in \cref{fig:arch-model}.%\carlos{move to some other section where we describe the experiments?} % The collision of a YuMi arm with a human triggers a safety stop that will disable the corresponding robot arm. With the standard variant of the robot control architecture using both arms, the robot would not be able to complete the task. Similarly, humans can obstruct the light sources, which makes operating with a camera unstable. We captured this model using the TOMASys ontology to build the knowledge base for the meta-controller. 
The knowledge base contains reusable tactics that can be reused across missions and systems. In the context of the dual-arm manipulator we developed the following tactics:
\emph{(i) reconfiguration tactic that aims to recover a function by selecting alternative function design;
%identify when a system error was identified and select the best alternative function design; 
(ii) tactic to identify and fix a broken component.}


%\subsubsection*{Runtime adaptation}
% For \emph{monitoring} we developed a proof of concept \emph{rosgraph\textunderscore monitor} that allowed mapping component errors in the deployed configurations to the corresponding architectural variant.  For \emph{execution} (reconfiguration) we developed a proof of concept \emph{rosgraph\textunderscore manipulator} mapping of configurations to basic actions that reconfigure the system by killing and launching the relevant ROS nodes.  For \emph{analysis and planning} we used the MROS meta-controller as a re-usable component.

\subsubsection{Mobile Robot Navigating in a Factory}
 %We implemented 30 different configurations of the system. 

%\subsubsection*{Models for Design}

We use the RosModels to model 27 different variants (\emph{i.e.} navigation stack configurations.) The RosModel tools allow to manually specify %the definition of a specific
the configuration for an existing ROS node. We created 27 different models that represent the possible configurations of \emph{move\_base}.  The variations respond to the combinations of different values of the \textit{move\_base} parameters, that have an impact on the behaviour of the navigation in terms of safety and energy consumption. As it is usual practice in robotics developments with ROS, we configured the components in the navigation stack with the intention to maximize the quality levels delivered for our particular use case, in this case in terms of performance, safety and energy.

%\subsubsection*{Runtime adaptation}
For runtime step R1 \emph{monitoring}, we developed observer models for safety and component failure.  Safety at run-time was modeled based on the collision risk\,\cite{chung2009safe}.  In this regard, we calculate a breaking distance of the robot before hitting an obstacle \emph{d\_break} and the distance from the current location of the robot to the closest obstacle in its direction $P$.  If the robot is at least \emph{d\_break} distance from the closest obstacle, runtime safety is always 1. As the robot approaches the closest obstacle, safety at run-time is computed as $\nicefrac{P}{\text{\emph{d\_break}}}$. 
%Energy at run-time was computed based on a energy model that simulates the power consumption of a robot. The energy model computes the instantaneous \emph{power\_load} of the robot using a set of information like current controller frequency, velocity, acceleration etc.
\looseness=-1

For runtime steps R2 and R3 \emph{analyze and plan} we used the MROS Meta-controller, as a re-usable component. In this context, we extended our knowledge base with a new reusable tactic \emph{to identify and fix violation of a system quality}. To generate the runtime model (K) we developed:
%
\begin{itemize}

  \item \emph{A navigation ontology} containing a minimal domain-specific model for navigation, that is elements to model the quality attributes safety, energy and performance, and associated adaptation rules in SWRL rules. 

    %\todo{remove this???<! --}, for example Rule 7 \carlos{add QAsafety or QAenergy rule from Protege as an equation or figure}\todo{ --> }

  \item \emph{A simple model-to-model transformation} to automatically generate the Knowledge Based from the RosSystem files and the TOMASys and navigation ontologies.

\end{itemize}


%
For \emph{execution}, we generalized and automated the ad-hoc solution developed for D1 using the RosModel tooling. This allows to automatically generate the available reconfiguration actions for the application architecture as \emph{ROS launch files} that can be used by the \emph{rosgraph\textunderscore manipulator}.
%developed for the first use case.



%with  minimal  modification  to  the  knowledge concepts  and  adaptation  logic.  
%Extensibility  is  a  measure of  the  ability  to  extend  a  system  and  the  level  of  effortr equired  to  implement  the  extension.  We  have  measuredas  a  cost  for  extending  our  system  at  knowledge  level  byadding/instantiating new concepts in the knowledge model

%the following RQ: \emph{Can model-based intelligent reconfiguration improve mission performance for robot systems?
%Can it address component failures at runtime? Can it manage quality concerns at runtime?}
%First, we demonstrate 
%demonstrate the usefulness of the Metacontrol framework in improving mission performance for robot systems by addressing component failures and quality concerns at runtime.


==> validation.tex <==
%In order to ensure a comprehensive and consistent experiment setup, we follow the Goal-Question-Metric method\,\cite{caldiera1994goal}.
%Our \emph{goal} is to \emph{Analyze 









%Proven by applying the MROS to the ABB case (early proof of concept) and later to the navigation case


%\looseness=-1
%in two factory scenarios.} 
%We refine this goal into the following Research Questions (our \textbf{RQ2}): \emph{Can model-based intelligent reconfiguration improve mission performance for robot systems? Can it address component failures at runtime? Can it manage quality concerns at runtime?}

%\subsection{Feasibility Study}



\section{Runtime adaptation feasibility}\label{lbl:feasibility}
We designed a systematic experimental setup to \emph{analyze the implementation of MROS with respect to its management of component failures and quality attribute concerns at runtime.}  In this context, we demonstrate how the Meta-control framwork is addressing component failures and quality concerns at runtme. We perform an investigation on how the MROS reconfiguration improves mission performance for robot systems by addressing functional and non-functional concerns.
%component failures and quality concerns at runtime.

We use two different robotic systems to validate MROS: the dual arm mobile manipulator discussed in the Introduction %(Section~\ref{sec:yumi}) 
and a mobile robot navigating in a factory (Section~\ref{sec:mob_factory}.\@  Both case studies are based on realistic applications for autonomous robots, concretely healthcare and manufacturing applications for mobile manipulators\,\cite{ABB-2019} with strong requirements. Mobile manipulation robots are designed to operate in semi-structured environments, such as a warehouse, a factory floor, and a healthcare facility.  Such environments keep changing dynamically. For example, the floor plan might change, some areas might be shared with humans and/or  other robots, etc.
This context variability demands varying configurations of the robot control architecture and appropriate methods to address functional and non-functional requirements.





%\subsection*{Management of component failures at runtime}
%In this section, we demonstrate how the MROS framework addresses component failures at run-time. 
%The experimental setup involved: (i) a dual-arm mobile manipulator, consisting of a ABB YuMi mounted on a Ridgeback omnidirectional platform and an Intel Real sense camera (\cref{sec:yumi}) and (ii) a mobile robot navigating in a factory scenario.

%We focus on performance of the different control schemes in different operational contexts as a key non-functional property here.  There are three scenarios:
%
%\begin{itemize}
 %   \item Scenario 1: workstation tag is not detected (a dual-arm manipulator).
  %  \item Scenario 2: manipulator can operate with only one arm (a dual-arm manipulator).
   % \item Scenario 3: laser sensor fails (a mobile robot).
%\end{itemize}
%
%The first scenario aims to demonstrate the MROS ability to recover a function that requires multiple components. The second and third scenario demonstrate the MROS controller's ability to recover from an error.

%by realising an alternative set of functions to perform the task goal with degraded performance.


%\subsection*{Management of Quality Attributes}
\subsection{Experimental Setup}\label{lbl:expDesign}
\input{componentfailures}
\input{experimentalsetup}

